Conditional independence by typing

A central goal of probabilistic programming languages (PPLs) is to separate modelling from inference. However, this goal is hard to achieve in practice. Users are often forced to re-write their models in order to improve efficiency of inference or meet restrictions imposed by the PPL. Conditional independence (CI) relationships among parameters are a crucial aspect of probabilistic models that capture a qualitative summary of the specified model and can facilitate more efficient inference. We present an information flow type system for probabilistic programming that captures conditional independence (CI) relationships, and show that, for a well-typed program in our system, the distribution it implements is guaranteed to have certain CI-relationships. Further, by using type inference, we can statically deduce which CI-properties are present in a specified model. As a practical application, we consider the problem of how to perform inference on models with mixed discrete and continuous parameters. Inference on such models is challenging in many existing PPLs, but can be improved through a workaround, where the discrete parameters are used implicitly, at the expense of manual model re-writing. We present a source-to-source semantics-preserving transformation, which uses our CI-type system to automate this workaround by eliminating the discrete parameters from a probabilistic program. The resulting program can be seen as a hybrid inference algorithm on the original program, where continuous parameters can be drawn using efficient gradient-based inference methods, while the discrete parameters are inferred using variable elimination. We implement our CI-type system and its example application in SlicStan: a compositional variant of Stan.

==> sections/abstract__.tex <==


Probabilistic programming languages (PPLs) often restrict the range of supported models, so as to make Bayesian inference feasible. For example, the Stan language uses an efficient gradient-based algorithm, by allowing only models where the posterior is a differentiable function over continuous parameters. Hence, models with discrete parameters cannot be used in Stan --- one of the main criticisms of the language. 
A workaround exists: users can work with discrete parameters \textit{implicitly}, by marginalising them out,
%of the target density, 
and carefully rearranging the program to re-draw them.
%from them using the provided random number generators. 
This task can be tedious and error-prone even for experienced users.

We introduce a source-to-source semantics-preserving transformation that automates marginalisation. The transformation uses a novel information-flow type system to capture conditional independence relationships,  marginalises out discrete parameters via variable elimination (VE), and appropriately draws them again.  
%
%The transformation takes a probabilistic program with discrete parameters and transforms it to a program without discrete parameters, by marginalizing them out using variable elimination (VE) and appropriately drawing them again. 
% The resulting program can be executed using Stan's standard HMC algorithm. 
Running the resulting program can be seen as running a hybrid inference algorithm on the original program, 
where continuous parameters are drawn using efficient gradient-based inference, while the discrete parameters are drawn using VE.


% We present a source-to-source semantics-preserving transformation, which uses our CI-type system to automate this workaround by eliminating the discrete parameters from a probabilistic program. 
% We do that using a novel information flow type system for probabilistic programming that captures conditional independence (CI) relationships,

We implement our approach in SlicStan: a compositional variant of Stan.\footnotemark We compare our static transformation to the run-time marginalisation strategy of NumPyro. Our method outperforms NumPyro on a range of standard models with mixed discrete and continuous parameters. 

\footnotetext{The implementation is available at 
<link anonymised for submission>.}
%\url{https://github.com/mgorinova/SlicStan}.}


\begin{comment}

A central goal of probabilistic programming languages (PPLs) is to separate modelling from inference. However, this goal is hard to achieve in practice. Users are often forced to re-write their models in order to improve efficiency of inference or meet restrictions imposed by the PPL. Conditional independence (CI) relationships among parameters are a crucial aspect of probabilistic models that captures a qualitative summary and can facilitate more efficient inference. 

We present an information flow type system for probabilistic programming that captures conditional independence (CI) relationships, and show that, for a well-typed program in our system, the distribution it implements is guaranteed to have certain CI-relationships. Further, by using type inference, we can statically \emph{deduce} which CI-properties are present in a specified model.

As a practical application, we consider the problem of how to perform inference on models with mixed discrete and continuous parameters. Inference on such models is challenging in many existing PPLs,  but can be improved through a workaround, where the discrete parameters are used \textit{implicitly}, at the expense of manual model re-writing. We present a source-to-source semantics-preserving transformation, which uses our CI-type system to automate this workaround by eliminating the discrete parameters from a probabilistic program. The resulting program can be seen as a hybrid inference algorithm on the original program, where continuous parameters can be drawn using efficient gradient-based inference methods, while the discrete parameters are drawn using variable elimination.

We implement our CI-type system and its example application in SlicStan: a compositional variant of Stan.\footnotemark

\footnotetext{The implementation is available at \url{https://github.com/mgorinova/SlicStan}.}

\end{comment}



==> sections/extended_examples.tex <==
\newpage
\section{Examples} \label{ap:examples}

\subsection{An extended HMM example} \label{ap:hmm}

This section works through a full example, showing the different steps of our approach. All results (intermediate and final) are as output by our preliminary implementation, up to formatting changes.

We consider the HMM model from earlier (Program D, \autoref{sec:application}), but reformulated to include transformed parameters:

\begin{lstlisting}
real phi0 ~ beta(1, 1);
real theta0 ~ beta(1, 1); 

int<2> z1 ~ bernoulli(theta0);
real theta1 = theta0 * z1 + (1 - theta0) * (1 - z1);
int<2> z2 ~ bernoulli(theta1);
real theta2 = theta0 * z2 + (1 - theta0) * (1 - z2);
int<2> z3 ~ bernoulli(theta2);

real phi1 = phi0 * z1 + (1 - phi0) * (1 - z1);
real phi2 = phi0 * z2 + (1 - phi0) * (1 - z2);
real phi3 = phi0 * z3 + (1 - phi0) * (1 - z3);

data real y1 ~ normal(phi1, 1);
data real y2 ~ normal(phi2, 1);
data real y3 ~ normal(phi3, 1);

real gentheta = theta1 * z3 + (1 - theta1) * (1 - z3);
int genz ~ bernoulli(gentheta);
\end{lstlisting}

The type levels of each variable are as defined by $\Gamma$:
\begin{align*}
	\Gamma = \{ &y_{1,2,3} : (\kw{real}, \lev{data}), \\
	& \phi_0 : (\kw{real}, \lev{model}), \theta_{0,1,2} : (\kw{real}, \lev{model}), \\
	& \phi_{1,2,3} : (\kw{real}, \lev{model}), z_{1,2,3} : (\kw{int<2>}, \lev{model}), \\
	& gen\theta : (\kw{real}, \lev{genquant}), genz : (\kw{int<2>}, \lev{genquant})\}
\end{align*}

The variables we are interested in transforming are $z_1, z_2$ and $z_3$: these are the $\lev{model}$-level discrete parameters of the model. The variable $\mathrm{genz}$ is already at $\lev{genquant}$ level, so we can sample this with ancestral sampling (no need for automatic marginalisation).

\subsubsection{Eliminating $z_1$}

\subsubsection{Standard shredding: $S \shred S_{D}, S_{M}, S_{Q}$} ~ 

Firstly, we separate out the parts of the program, which depend on discrete parameters \textit{generatively}. That is any part of the program which would be in generated quantities w.r.t. the original program. In our case, this includes the last two lines in $S$. This would also include the \kw{gen} parts of the transform program, that draw discrete parameters as generated quantities. 

Thus, $S \shred S_{D}, S_{M}, S_{Q}$, where $S_{D}$ is empty,
\lstinline!$S_{Q} = $ theta1*z3 + (1-theta1) * (1-z3); genz ~ bernoulli(gentheta)!, and $S_M$ is the rest of the program. 

\subsubsection{Conditional independence shredding: $S_M \shred[\Gamma_M] S_1, S_2, S_3$} ~ 

In the next step, we want establish a conditional independence relationship $z_1 \mid A \mid \mathbf{y}, \phi_0, \theta_0, B$, where $A, B$ is a partitioning of the rest of the discrete parameters in the model: $\{z_2, z_3\}$. 
We derive a new, $\typingspecial$ typing environment $\Gamma_M$, using $\Gamma \xrightarrow{z} \Gamma_M$:
\begin{align*} 
	\Gamma_M = \{ & y_{1,2,3} : (\kw{real}, \lev{l1}), \phi_0 : (\kw{real}, \lev{l1}), \theta_0: (\kw{real}, \lev{l1}), \\
	& z_{1} : (\kw{int<2>}, \lev{l2}), z_2 : (\kw{int<2>}, \lev{?}), z_3 : (\kw{int<2>}, \lev{?}) \\
	& \theta_{1,2} : (\kw{real}, \lev{?}), \phi_{1,2,3} : (\kw{real}, \lev{?})\}
\end{align*}

Here, we use the notation $\lev{?}$ for a type placeholder, which will be inferred using type inference.  

The optimal $\Gamma_M$ under the type inference soft constraint $\lev{l3} < \lev{l1} < \lev{l2}$ such that $\Gamma_M \typingspecial S_M : \lev{l1}$ is such that the levels of $\theta_{1}$ and $\phi_{1}$ are \lev{l2}, $z_2$ is \lev{l1} and $\theta_2, \phi_2$ and $\phi_3$ are \lev{l3}.
Shredding then gives us
$S_M \shred[\Gamma_M] S_1, S_2, S_3 $,
%
where: 
\begin{lstlisting}
$S_1 = $ phi0 ~ beta(1, 1);
		 theta0 ~ beta(1, 1);

$S_2 = $ z1 ~ bernoulli(theta0);
		 theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
		 z2 ~ bernoulli(theta1);
		 phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));
		 y1 ~ normal(phi1, 1);

$S_3 = $ theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
		 z3 ~ bernoulli(theta2);
		 phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));
		 phi3 = (phi0 * z3 + (1 - phi0) * (1 - z3));
		 y2 ~ normal(phi2, 1);
		 y3 ~ normal(phi3, 1);
\end{lstlisting}

\subsubsection{Putting everything together}~
\vspace{6pt}

Having rearranged the program into suitable sub-statements, we use \ref{Elim Gen} to get:
\begin{align*}
	\Gamma' = \{ &y_{1,2,3} : (\kw{real}, \lev{data}), \phi_0 : (\kw{real}, \lev{model}), \\
	& \theta_1 : (\kw{real}, \lev{genquant}), \theta_{0,2} : (\kw{real}, \lev{model}), \\
	& \phi_1 : (\kw{real}, \lev{genquant}), \phi_{2,3} : (\kw{real}, \lev{model}), \\
	& z_{1} : (\kw{int}, \lev{genquant}), z_{2,3} : (\kw{int<2>}, \lev{model}), \\
	& gen\theta : (\kw{real}, \lev{genquant}), genz : (\kw{int<2>}, \lev{genquant})\}
\end{align*}

And the program:

\begin{lstlisting}
phi0 ~ beta(1, 1);
theta0 ~ beta(1, 1);

f1 = $\phi$([int<2> z2]){
	elim(int<2> z1){
		z1 ~ bernoulli(theta0);
		theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
		z2 ~ bernoulli(theta1);
		phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));
		y1 ~ normal(phi1, 1);
	}
}
factor(f1[z2]);

theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
z3 ~ bernoulli(theta2);
phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));
phi3 = (phi0 * z3 + (1 - phi0) * (1 - z3));
y2 ~ normal(phi2, 1);
y3 ~ normal(phi3, 1);

gen(int z1){
	z1 ~ bernoulli(theta0);
	theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
	z2 ~ bernoulli(theta1);
	phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));
	y1 ~ normal(phi1, 1);
}
theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));

gentheta = (theta0 * z3 + (1 - theta0) * (1 - z3));
genz ~ bernoulli(gentheta);
\end{lstlisting}

\subsubsection{Eliminating $z_2$}

We apply the same procedure to eliminate the next variable. 
The variable $z_1$ is no longer a \lev{model}-level parameter, thus the only neighbouring parameter of $z_2$ is $z_3$. Note also that the computation of the factor $f_1$ does not include any free discrete parameters (both $z_1$ and $z_2$ are local to the computation due to $\kw{elim}$ and $\phi$). Thus, we do not need to include the computation of this factor anywhere else in the program (it does not get nested into other computations).

After rearranging, we get:
\begin{lstlisting}
phi0 ~ beta(1, 1);
theta0 ~ beta(1, 1);

f1 = $\phi$([int<2> z2]){
	elim(int<2> z1){
		z1 ~ bernoulli(theta0);
		theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
		z2 ~ bernoulli(theta1);
		phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));
		y1 ~ normal(phi1, 1);
	}
}

f2 = $\phi$([int<2> z3]){
	elim(int<2> z2){
		factor(f1[z2]);
		theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
		z3 ~ bernoulli(theta2);
		phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));
		y2 ~ normal(phi2, 1);
	}
}

factor(f2[z3]);
phi3 = (phi0 * z3 + (1 - phi0) * (1 - z3));
y3 ~ normal(phi3, 1);

gen(int z2){
	factor(f1[z2]);
	theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
	z3 ~ bernoulli(theta2);
	phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));
	y2 ~ normal(phi2, 1);
}
theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));

gen(int z1){
	z1 ~ bernoulli(theta0);
	theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
	z2 ~ bernoulli(theta1);
	phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));
	y1 ~ normal(phi1, 1);
}
theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));

gentheta = (theta0 * z3 + (1 - theta0) * (1 - z3));
genz ~ bernoulli(gentheta);
\end{lstlisting}

\subsubsection{Eliminating $z_3$}

Finally, we eliminate $z_3$, which is the only discrete \lev{model}-level parameter left in the program. Thus, $z_3$ has no neighbours and $f_3$ is of arity 0 --- it is a real number instead of a vector.  

The final program generated by our implementation is:
\begin{lstlisting}
phi0 ~ beta(1, 1);
theta0 ~ beta(1, 1);

f1 = $\phi$(int<2> z2){
	elim(int<2> z1){
		z1 ~ bernoulli(theta0);
		theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
		z2 ~ bernoulli(theta1);
		phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));
		y1 ~ normal(phi1, 1);
	}
}
f2 = $\phi$(int<2> z3){
	elim(int<2> z2){
		factor(f1[z2]);
		theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
		z3 ~ bernoulli(theta2);
		phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));
		y2 ~ normal(phi2, 1);
	}
}
f3 = $\phi$(){
	elim(int<2> z3){
		factor(f2[z3]);
		phi3 = (phi0 * z3 + (1 - phi0) * (1 - z3));
		y3 ~ normal(phi3, 1);
	}
}

factor(f3);

gen(int z3){
	factor(f2[z3]);
	phi3 = (phi0 * z3 + (1 - phi0) * (1 - z3));
	y3 ~ normal(phi3, 1);
}
phi3 = (phi0 * z3 + (1 - phi0) * (1 - z3));

gen(int z2){
	factor(f1[z2]);
	theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
	z3 ~ bernoulli(theta2);
	phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));
	y2 ~ normal(phi2, 1);
}
theta2 = (theta0 * z2 + (1 - theta0) * (1 - z2));
phi2 = (phi0 * z2 + (1 - phi0) * (1 - z2));

gen(int z1){
	z1 ~ bernoulli(theta0);
	theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
	z2 ~ bernoulli(theta1);
	phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));
	y1 ~ normal(phi1, 1);
}
theta1 = (theta0 * z1 + (1 - theta0) * (1 - z1));
phi1 = (phi0 * z1 + (1 - phi0) * (1 - z1));

gentheta = (theta0 * z3 + (1 - theta0) * (1 - z3));
genz ~ bernoulli(gentheta);
\end{lstlisting}


==> sections/new_background.tex <==

\section{SlicStan: Extended syntax and semantics} \label{sec:background}
SlicStan \cite{SlicStanPOPL} is a Stan-like probabilistic programming language.
Compared to Stan, it adds extra compositionality by dropping the requirement that programs be block-structured.
SlicStan uses type inference in an information-flow type system
\cite{DBLP:journals/jcs/VolpanoIS96, % first one ADG knows of
      DBLP:conf/popl/AbadiBHR99, % shows connection to program slicing/shredding
      DBLP:conf/esop/GordonRSBRGT15} % prior work on information flow for PP
to automatically rearrange the program into parts roughly corresponding to the blocks-structure of Stan: pre-processing (data), model and post-processing (generated quantities).
Originally, this \textit{shredding} was developed to compile SlicStan to Stan.
In this paper, that it can be used, more generally, to automatically compile to an efficient program-specific inference scheme.


Like Stan, SlicStan is imperative and allows for deterministic assignment, for-loops, if-statements, probabilistic assignment, and factor-statements.
One contribution of this work is that we present an updated version of SlicStan.
For example, we expand on the meaning of $\sim$ in SlicStan. 
In the original SlicStan paper \cite{SlicStanPOPL}, a statement such as $x \sim \normal(0, 1)$ was understood simply as a syntactic sugar for $\kw{factor}(\normal(x \mid 0, 1))$. This means those statements were always interpreted as part of the model block in Stan. 
In our updated version of SlicStan, the semantics of $x \sim \normal(0, 1)$ remains \emph{equivalent} to that of $\kw{factor}(\normal(x \mid 0, 1))$, however it could be \emph{implemented} differently depending on the context. In particular, $x \sim \normal(0, 1)$ could be implemented as a simple call to a random number generator in Stan, $x = \normal_{rng}(0, 1)$, like in the example below.

\begin{figure*}
\vspace{-10pt}
\begin{multicols}{3} 
\begin{lstlisting}
// Stan target program
data{ real x; }
parameters{ real $\mu$; }
model{ x $\sim$ normal($\mu$, 1); }
generated quantities{ 
	real x_pred = normal_rng($\mu$, 1); }
\end{lstlisting}	
	
\begin{lstlisting} 
    // SlicStan from POPL'19
    
    real $\mu$;
    data real x $\sim$ normal($\mu$, 1);
    real x_pred = normal_rng($\mu$, 1);

\end{lstlisting}	

\begin{lstlisting}
    // extended SlicStan
    
    real $\mu$;
    data real x $\sim$ normal($\mu$, 1);
    real x_pred $\sim$ normal($\mu$, 1);

\end{lstlisting}
\end{multicols} \vspace{-10pt}
\caption{Example of difference to previous version of SlicStan}
\end{figure*}

\noindent Treating $\sim$ statements differently based on context is very similar in spirit to existing effect-handling based PPLs like Edward2 and Pyro, where $\sim$ can be handled in different ways. However, in our case, this difference in treatment is determined statically, automatically, and only in the translation to Stan or another backend. 

In the rest of this section, we give the updated formal syntax, typing and semantics of SlicStan and describe shredding --- the procedure key to the translation of Stan / inference composition. 

\subsection{Syntax} \label{ssec:syntax}
SlicStan has the following types, programs, L-values,
statements, and expressions. We highlight the difference with \cite{SlicStanPOPL} with boxes.

\begin{display}[.50]{SlicStan Types:}
	\clause{\ell ::= \lev{data} \mid \lev{model} \mid \lev{genquant}}{level type}\\
	\clause{n\in\mathbb{N}}{size} \\
	\clause{\tau ::= \kw{real} \mid \kw{int} \mid \fbox{$\kw{int}\langle n \rangle$} \mid \tau [n]}{base type} \\
	\clause{T ::= (\tau,\ell)}{type}
\end{display}
\vspace{-5pt}
\begin{display}[.35]{SlicStan Program:}
	\clause{P ::= \Gamma,S}{program}
\end{display}
\vspace{-5pt}
\begin{display}[.35]{SlicStan L-Values:}
	\clause{L ::= x[E_1]\cdots[E_n]}{L-value}
\end{display}
\vspace{-5pt}
\begin{display}{SlicStan Typing Environments:}
	\clause{\Gamma ::= \{x_1\mapsto T_1,\ldots, x_n\mapsto T_n\}}{typing environment}
\end{display}

\vspace{-5pt}
\begin{display}[.35]{SlicStan Statements:}
	\Category{S}{statement}\\
	% \entry{(\tau,\ell)\,x;\,S}{declaration}\\
	\entry{L = E}{assignment}\\
	\entry{S_1; S_2}{sequence}\\
	\entry{\kw{for}(x\;\kw{in}\;E_1:E_2)\;S}{for loop} \\
	\entry{\kw{if}(E)\;S_1\,\kw{else}\;S_2}{if statement} \\
	\entry{\kw{skip}}{skip}\\
	\entry{\fbox{\kw{factor}(E)}}{{factor statement}} \\
	\entry{\fbox{$L \sim d(E_1, ..., E_n)$}}{sample statement}
\end{display}
\vspace{-5pt}
\begin{display}[.35]{SlicStan Expressions:}
	\Category{E}{expression}\\
	\entry{x}{variable}\\
	\entry{c}{constant}\\
	\entry{[E_1,...,E_n]}{array}\\
	\entry{E_1[E_2]}{array element}\\ 
	\entry{f(E_1,\dots,E_n)}{function call}\\
	\entry{\fbox{$[E \mid x~\kw{in}~E_1:E_2]$}}{{array comprehension}}\\
	\entry{\fbox{\kw{target}(S)}}{{evaluating a density}}
	% \Category{L}{L-value}\\[-12pt]
	% \entry{\;x[E_1]\cdots[E_n]}{}
\end{display}
\vspace{-5pt}

SlicStan programs consist of a pair $\Gamma,S$ of a \emph{typing environment} $\Gamma$
(a finite map which assigns global variables $x$ to their types $T$)
and a \emph{statement} $S$.
Following the usual style of declaring variables in C-like languages,
we informally present programs $\Gamma,S$ in examples
by sprinkling the type declarations of $\Gamma$
throughout the statement $S$.
For example, we write $\kw{data}~\kw{real}~x \sim~ \kw{normal}(0, 1)$ for the program 
$\{x\mapsto (\kw{real},\lev{data})\}, x \sim \kw{normal}(0, 1)$.
Sometimes, we will leave out types or write incomplete types in our examples.
In this case, we intend for the missing types to be determined using %our 
type inference. % algorithm. 

%We assume syntax for array comprehensions for clarity.
As we discuss in detail in \autoref{ssec:stanop}, a $\kw{factor}(E)$ statement can be read as
multiplying the current \emph{weight} of the program trace by the value of $E$.
Conversely, a $\kw{target}(S)$ expression initializes the weight to $1$
and returns the weight that is accumulated after evaluating $S$.
For example, if: \vspace{-4pt}
\begin{align*}
S &= \kw{x ~ normal(0,1); y = 2 * x; z ~ normal(y,1);} \\
&=  \kw{factor(normal_pdf(x|0,1)); y = 2 * x; factor(normal_pdf(z|y,1));}
\end{align*}
\noindent Then $\kw{target}(S)$ is semantically equivalent to \kw{normal_pdf(x|0,1) * normal_pdf(z|2 * x,1)}.

We extend the base types of the language of \cite{SlicStanPOPL} with $\kw{int}\langle n \rangle$, which denotes a positive integer constrained from above by an integer $n$. For example if $x$ is of type $\kw{int}\langle 2 \rangle$, then $x$ can only be 1 or 2. These types allow us to specify the support of discrete variables, and they can easily be extended to include both upper and lower bounds. %, where types can be constraint using the keywords \lstinline|upper| and \lstinline|lower|).
%
For the purpose of our typing rules, we treat $\kw{int}\langle n \rangle$ identically to $\kw{int}$. We only differentiate between these types in $\autoref{sec:application}$, where our transformation uses the size annotation to eliminate a discrete variable.




\subsection{Typing} \label{ssec:typing}

Types $T$ in SlicStan range over pairs $(\tau, \ell)$ of a base type $\tau$, and a level type $\ell$. The level types $\ell$ form a lattice $\left(\{\lev{data}, \lev{model}, \lev{genquant}\}, \leq \right)$, where $\lev{data} \leq \lev{model} \leq \lev{genquant}$.
We write $\bigsqcup_{i=1}^n \ell_i$ for the least upper bound of the levels $\ell_1,\ldots,\ell_n$.
We call variables of level $\lev{data}$ \emph{data (variables)}, 
of level $\lev{model}$ \emph{model parameters},
and of level $\lev{genquant}$ \emph{generated quantities}.
We refer to variables that are either of level $\lev{model}$ or $\lev{genquant}$ 
simply as \emph{parameters}.
Given a typing environment $\Gamma$,
we can consider the well-typedness of expressions and statements,
given the types assigned to variables by $\Gamma$.
The judgment $\Gamma \vdash E : (\tau, \ell)$ means that expression $E$ has type $\tau$ and reads only level $\ell$ and below.
The judgment $\Gamma \vdash S : \ell$ means that statement $S$ assigns only to level $\ell$ and above.
We write $\Gamma\vdash S$ as a shorthand for $\Gamma\vdash S:\lev{data}$.


The typing rules for expressions are those of \cite{SlicStanPOPL} with added rules 
for the two constructs of array comprehensions and $\kw{target}(S)$-expressions. 
The typing rules for statements are as in \cite{SlicStanPOPL}, with three differences (highlighted in boxes). \ref{Factor} and \ref{Sample} add typing rules for the now new language constructs $\kw{factor}(E)$ and $L \sim d(E_1, ..., E_n)$.
The language supports a finite number of 
built-in functions $f$ with type $\tau_1,\ldots,\tau_n\to \tau$ 
and (conditional) distributions $d\in\mathrm{Dist}(\tau_1,\ldots,\tau_n;\tau)$ over $\tau$ given values 
of types $\tau_1,\ldots,\tau_n$.

\begin{display}{Typing Rules for Expressions:}\scalebox{0.81}{\parbox{1.3\linewidth}{%
	\staterule{ESub}
	{ \Gamma \vdash E : (\tau,\ell) \quad \ell \leq \ell'}
	{ \Gamma \vdash E : (\tau,\ell') }\quad\quad%
	%
	\staterule{Var}
	{ }
	{ \Gamma, x:T \vdash x:T}\quad\quad%  
	%
	%\hquad
	\staterule{Const}
	{ \kw{ty}(c) = \tau }
	{ \Gamma \vdash c : (\tau,\lev{data}) }%
	
	%\hquad
	\staterule[($f: \tau_1,\dots,\tau_n \to \tau$)]
	{PrimCall}
	{ \Gamma \vdash E_i : (\tau_i,\ell_i) \quad \forall i \in 1..n}
	{ \Gamma \vdash f(E_1,\dots,E_n) : (\tau,\bigsqcup_{i=1}^n \ell_i )}\quad% 
	%
	\fbox{\staterule{Target}
	{\Gamma\vdash S :\ell''\quad \forall \ell' > \ell. \readset_{\Gamma \vdash \ell'}(S)=\emptyset \footnotemark}
	{\Gamma\vdash \kw{target}(S) : (\kw{real},\ell)}}\quad%
	%
	%
	%\\[\GAP]
	\staterule{ArrEl}
	{\Gamma \vdash E_1 : (\tau[n], \ell) \quad \Gamma \vdash E_2 : (\kw{int}, \ell)}
	{\Gamma \vdash E_1[E_2] : (\tau,\ell)}%
	%
    \qquad 
	\staterule{Arr}
	{\Gamma \vdash E_i : (\tau,\ell) \quad \forall i \in 1..n}
	{\Gamma \vdash [E_1,...,E_n] : (\tau [n],\ell)}%
	\\
	\squad
	\fbox{\staterule{ArrComp}
	{\Gamma\vdash E_1 : (\kw{int},\ell)\quad \Gamma\vdash E_2 : (\kw{int},\ell)\quad \Gamma, x:(\kw{int},\ell)\vdash E : (\tau,\ell)\quad x \notin \dom(\Gamma)}
	{\Gamma \vdash [E \mid x~\kw{in}~E_1:E_2] : (\tau[n],\ell)}}
}}
\end{display}

\footnotetext{We use $\ell' > \ell$ as a shorthand for $\ell \leq \ell' \wedge \neg \ell' \leq \ell $ }

%\begin{figure*}
\begin{display}{Typing Rules for Statements:}\scalebox{0.74}{\parbox{1.3\linewidth}{%
	\squad
	\staterule{SSub}
	{ \Gamma \vdash S : \ell' \quad \ell \leq \ell'}
	{ \Gamma \vdash S : \ell }\squad% %\quad
	%
	\staterule{Assign}
	{ \Gamma(L) = (\tau, \ell) \quad \Gamma \vdash E : (\tau,\ell)}
	{ \Gamma \vdash (L = E) : \ell }\squad% %\qquad 
	%
	\staterule{If}
	{ \Gamma \vdash E : (\kw{real},\ell) \quad \!\Gamma \vdash S_1\! :\! \ell \quad\! \Gamma \vdash S_2\! :\! \ell}
	{ \Gamma \vdash \kw{if}(E)\;S_1 \;\kw{else}\; S_2: \ell } %\qquad
	%
	\\
	\fbox{
	\staterule{Factor}
	{ \Gamma \vdash E : (\kw{real}, \lev{model})}
	{ \Gamma \vdash \kw{factor}(E) : \lev{model} }} %\qquad
	%
	%
	%
 	\fbox{
	\staterule{Seq}
	{ \Gamma \vdash S_1 : \ell \quad \Gamma \vdash S_2 : \ell \quad \shreddable(S_1, S_2)\,\wedge\, \generative(S_1, S_2)}
	{ \Gamma \vdash (S_1; S_2) : \ell }} %\qquad
	%
    %\\[\GAP]\squad
	\fbox{
	\staterule[($d\in \mathrm{Dist}(\tau_1,\dots,\tau_n ;\tau)$)]{Sample}
	{ \Gamma(L) = (\tau,\ell') \quad\! \Gamma \vdash E_i : (\tau_i, \ell), \,\, \forall i \in 1..n \quad\! \ell = \ell' \sqcup \lev{model}}
	{ \Gamma \vdash L \sim d(E_1, \dots, E_n) : \ell }} %\quad\!
	%
	%
	%\\[\GAP]\squad	
	\staterule{Skip}
	{ }
	{ \Gamma \vdash \kw{skip} : \ell } %\qquad
	%
	%\\[\GAP]\squad
	\staterule{For}
	{ \Gamma \vdash E_1 : (\kw{int},\ell) \quad \Gamma \vdash E_2 : (\kw{int},\ell) \quad \Gamma, x:(\kw{int}, \ell) \vdash S : \ell \quad x \notin \dom(\Gamma) \quad x \notin \assset(S)}
	{ \Gamma \vdash \kw{for}(x\;\kw{in}\;E_1:E_2)\;S : \ell } 
}}
\end{display}
%\end{figure*}


In these rules, we make use of the following definitions (see \autoref{ap:proofs} for precise definitions).
\begin{itemize}
	\item $\readset_{\Gamma \vdash \ell}(S)$: the set of variables $x$ that are read at level $\ell$ in $S$. %For example, if $y$ is of level $\ell$, then $x\in \readset_{\Gamma \vdash \ell}(y=x)$.
	\item $\assset_{\Gamma \vdash \ell}(S)$: the set of variables $x$ of level $\ell$ that have been assigned to in $S$.
	\item $\tildeset_{\Gamma\vdash \ell}(S)$: the set of variables $x$ of level $\ell$ that have been $\sim$-ed in $S$.
	\item $\asstildeset_{\Gamma\vdash \ell}(S)= \assset_{\Gamma\vdash \ell}(S)\cup \tildeset_{\Gamma\vdash \ell}(S)$ %: the set of variables $x$ of level $\ell$ that have been assigned to or $\sim$-ed in $S$.
\end{itemize}

\begin{definition}[Shreddable seq]~ $\shreddable(S_1, S_2) \deq  \forall \ell_1,\ell_2. (\ell_2 < \ell_1) \implies \readset_{\Gamma \vdash \ell_1}(S_1) \cap \assset_{\Gamma \vdash \ell_2}(S_2) = \emptyset$
\end{definition}
The intention in SlicStan is that statements of level $\ell$ are executed before those of 
$\ell'$ if $\ell<\ell'$.
In order to follow that implementation strategy without reordering possibly non-commutative pairs of statements, we impose the condition $\shreddable(S_1, S_2)$ when we sequence $S_1$ and $S_2$.
\begin{definition}[Generative seq] ~ $\generative(S_1, S_2) \deq  \forall \ell\neq \lev{model}.\, \tildeset_{\Gamma\vdash \ell}(S_1)\cap \asstildeset_{\Gamma\vdash \ell}(S_2)=\emptyset \wedge \asstildeset_{\Gamma\vdash \ell}(S_1)\cap \tildeset_{\Gamma\vdash \ell}(S_2)=\emptyset$
\end{definition}
To be able to read $x\sim \normal(0,1)$, depending on the context, either as a probabilistic assignment to $x$
or as a density contribution, we impose the condition $\generative(S_1, S_2)$
when we sequence $S_1$ and $S_2$.


\subsection{Operational Semantics of SlicStan Statements} \label{ssec:stanop}
In this paper, we use a modified version of the semantics given in \citet{SlicStanPOPL}.
We extend the call-by-value operational semantics given in that paper, and derive a more equational form that also includes the generated quantities. 

We define a standard big-step operational semantics for SlicStan expressions and statements:
\begin{display}[.2]{Big-step Relation}
	\clause{ (s, E) \Downarrow V }{expression evaluation} \\
	\clause{ (s, S) \Downarrow (s',w)}{statement evaluation} 
\end{display}
Here, $s$ and $s'$ are \emph{states}, $V$ is a \emph{value} and $w\in \weights$ is a \emph{weight}.
Our statements can read and write the state with arbitrary destructive updates.
The weight can be thought of as a bit of 
state that stores a positive real value which only 
gets accessed by multiplying it with the value of an expression $E$, through the use of 
$\kw{factor}(E)$-statements.
It can only be read through a $\kw{target}(S)$-statement
which initialises the weight to $1$, evaluates the statement $S$
and returns the final weight.

Formally, states and values are defined as follows.
% If $\Gamma = x_1:T_1, \dots, x_n:T_n$ let a \emph{valuation} of $\Gamma$
% be a sequence of bindings $x_1=V_1,\dots,x_n=V_n$ where each $V_i$ is a value of type $\tau_i$ where $T_i=(\tau_i,\ell_i)$.
\begin{display}[0.4]{Values and States:}
	\Category{V}{value}\\
	\entry{c}{constant}\\
	\entry{[V_1,\dots,V_n]}{array}\\
	\clause{s ::= x_1 \mapsto V_1, \dots, x_n \mapsto V_n \quad}{state}
\end{display}


In the rest of the paper, we use the notation for states $s = x_1 \mapsto V_1, \dots, x_n \mapsto V_n$:
\begin{itemize}
	\item $s[x \mapsto V]$ is the state $s$, but where the value of $x$ is updated to $V$ if $x \in \dom(s)$, or the element $x \mapsto V$ is added to $s$ if $x \notin \dom(s)$.
	%\begin{itemize}
	%	\item $s[x \mapsto V] = x_1 \mapsto V_1, \dots, x_i \mapsto V, \dots, x_N \mapsto V_N$ if $x = x_i$ for some $n \in 1 .. n$, or
	%	\item $s[x \mapsto V] = x_1 \mapsto V_1, \dots, x_i \mapsto V_i, x \mapsto V$ if $\forall i \in 1 .. n. x \neq x_i$.  
	%\end{itemize}
	\item $s[-x]$ is the state s, but where $x$ is removed from the domain of $s$ (if it were present).
	%\begin{itemize}
	%	\item $s[-x] = x_1 \mapsto V_1, \dots, x_{i-1} \mapsto V_{i-1}, x_{i+1} \mapsto V_{i+1} \dots, x_n \mapsto V_n$ if $x = x_i$ for some $i \in 1..n$, or
	%	\item $s[-x] = s$ if $x \neq x_i \forall i \in 1..n$.  
	%\end{itemize}
\end{itemize}

%\vspace{12pt} %FLAG space

We also define lookup and update operations on values:
\begin{itemize}
	\item If $U$ is an $n$-dimensional array value for $n \geq 0$
	and $c_1$, \dots, $c_n$ are suitable indexes into $U$,
	then the \emph{lookup} $U[c_1]\dots[c_n]$ is the value in $U$ indexed by $c_1$, \dots, $c_n$.
	\item If $U$ is an $n$-dimensional array value for $n \geq 0$
	and $c_1$, \dots, $c_n$ are suitable indexes into $U$,
	then the (functional) \emph{update} $U[c_1]\dots[c_n] := V$ is the array that is the same as $U$ except that the
	value indexed by $c_1$, \dots, $c_n$ is $V$.
\end{itemize}



The relation $\Downarrow$ is deterministic but partial, as we do not explicitly handle error states.
The purpose of the operational semantics is to define a density function in \autoref{ssec:standen}, and any errors lead to the density being undefined.
The big-step semantics is defined as follows.
\vspace{3pt}

\begin{display}{Operational Semantics of Expressions:}
\scalebox{0.81}{\parbox{1.3\linewidth}{
	\squad	
	\staterule{Eval Const}
	{ }
	{ (s, c) \Downarrow c }\quad
	%
	\staterule{Eval Var}
	{ V = s(x)  \quad x \in \dom(s)}
	{ (s, x) \Downarrow V  }\quad
	%
	\staterule{Eval Arr}
	{ (s, E_i) \Downarrow V_i \quad \forall i \in 1.. n }
	{ (s, [E_1, \dots, E_n]) \Downarrow [V_1, \dots, V_n]}\qquad	
	
	\staterule{Eval ArrEl}
	{ (s, E_1 \Downarrow V) \quad (s, E_2 \Downarrow c)}
	{ (s, E_1[E_2]) \Downarrow V[c]}\quad
	%
	\staterule[\footnotemark]{Eval ArrComp}
	{ (s, E_1) \Downarrow n \quad (s, E_2) \Downarrow m \quad (s, E[i/x]) \Downarrow V_i, \forall i\in n..m }
	{ (s, [E \mid x~\kw{in}~E_1:E_2]) \Downarrow [V_{n},\ldots, V_{m}] }\qquad
	
	\staterule{Eval PrimCall}
	{ (s, E_i) \Downarrow V_i \quad  i \in 1 \dots n \quad V = f(V_1, \dots, V_n)\footnotemark}
	{ (s, f(E_1, \dots, E_n)) \Downarrow V}\qquad
	%
	\staterule{Eval Target}
	{ (s, S) \Downarrow (s', w)}
	{ (s, \kw{target}(S)) \Downarrow w}}}
\end{display}

\footnotetext[2]{$f(V_1, \dots, V_n)$ means applying the built-in function $f$ on the values $V_1, \dots, V_n$.}
\footnotetext{Here, we write $E[E'/x]$ for the usual capture avoiding substitution of $E'$ for $x$ in $E$.}
%
%\vspace{-3pt}
%
%\adg{Perhaps a single-step semantics would give us more information, as it can explicitly represent the errors that are prevented by the type system.}

\begin{figure*}
\begin{display}{Operational Semantics of Statements:}

	\staterule[~(where $L=x[E_1{]}\dots[E_n{]}$)]{Eval Assign}
	{ (s,E_i) \Downarrow V_i \quad \forall i \in 1..n \quad (s,E) \Downarrow V \quad
		U = s(x) \quad
		U' = (U[V_1]\dots[V_n] := V) }
	{ (s, L=E) \Downarrow (s[x \mapsto U'], 1)}\quad
	
	\staterule{Eval Skip}
	{ }
	{ (s, \kw{skip}) \Downarrow (s, 1) }\quad
	
	\staterule{Eval Seq}
	{ (s, S_1) \Downarrow (s', w) \quad (s', S_2) \Downarrow (s'', w')}
	{ (s, S_1;S_2) \Downarrow (s'', w * w')}\squad
	
	
	\\[\GAP]\squad
	\staterule{Eval ForFalse}
	{ (s, E_1) \Downarrow c_1 \quad (s, E_2) \Downarrow c_2 \quad c_1 > c_2}
	{ (s, \kw{for}(x\;\kw{in}\;E_1:E_2)\;S) \Downarrow (s, 1) } \squad

	
	\staterule{Eval ForTrue}
	{ \{(s, E_i) \Downarrow c_i\}_{i=1,2} \quad c_1 \leq c_2 \quad (s[x \mapsto c_1], S) \Downarrow (s', w) \quad (s'[-x], \kw{for}(x\;\kw{in}\;(c_1+1):c_2)\;S) \Downarrow (s'', w')}
	{ (s, \kw{for}(x\;\kw{in}\;E_1:E_2)\;S) \Downarrow (s'', w * w') } \qquad
	
	\\[\GAP]\squad
	\staterule{Eval IfTrue}
	{ (s, E) \Downarrow c\neq 0.0 \quad (s, S_1) \Downarrow (s', w)}
	{ (s, \kw{if}(E)\; S_1\; \kw{else}\; S_2) \Downarrow (s', w)}\quad
	
	\staterule{Eval IfFalse}
	{ (s, E) \Downarrow 0.0 \quad (s, S_2) \Downarrow (s', w)}
	{ (s, \kw{if}(E)\; S_1\; \kw{else}\; S_2) \Downarrow (s', w)}\quad


    \\[\GAP]\squad
    \staterule{Eval Factor}
	{ (s, E) \Downarrow V }
	{ (s, \kw{factor}(E)) \Downarrow (s, V)}\quad
	
	\staterule{Eval Sample}
	{ (s, L) \Downarrow V \quad (s, E_i) \Downarrow V_i, \forall 1\leq i \leq n\quad V' =d(V| V_1,\ldots, V_n)\footnotemark  }
	{ (s, L \sim d(E_1, \ldots, E_n)) \Downarrow (s, V') }
\end{display}

\end{figure*}

\footnotetext[1]{By $d(V|V_1,\ldots,V_n)$, we mean the result of evaluating the intended built-in conditional distribution $d$ on $V,V_1,\ldots,V_n$.}

The design of the type system ensures that information 
can flow from a level $\ell$ to a higher one $\ell'\geq \ell$,
but not a lower one $\ell'<\ell$: a noninterference result.
To state this formally, we introduce the notions of
\emph{conformance between a state $s$ and a typing environment $\Gamma$} and
\emph{$\ell$-equality} of states.

We define a conformance relation on states $s$ and typing environments $\Gamma$. A state $s$ \emph{conforms} to an environment $\Gamma$, whenever $s$ provides values of the correct types for the variables used in $\Gamma$:

\begin{display}[-0.03]{Conformance Relation:}
	\clause{ s \models \Gamma }{state $s$ conforms to environment $\Gamma$}
\end{display}
\begin{display}[.2]{Rule for the Conformance Relation:}
	\quad
	\staterule{Stan State}
	{ V_i \models \tau_i \quad \forall i \in I}
	{(x_i \mapsto V_i)^{i \in I} \models (x_i : \tau_i)^{i \in I}}
\end{display}

Here, $V \models \tau$ denotes that the value $V$ is of type $\tau$, and has the following definition:
\begin{itemize}
	\item $c \models \kw{int}$, if $c \in \mathbb{Z}$, and $c \models \kw{real}$, if $c \in \mathbb{R}$. 
	% \item \st{$[V_1,\dots,V_n] \models \tau[n]$, if $\forall i \in 1\dots n. V_i \models \tau$.}
	\item $[V_1,\dots,V_n] \models \tau[m]$, if $\forall i \in 1\dots n. V_i \models \tau$. 
\end{itemize}


\begin{definition}[$\ell$-equal states]~\\ Given a typing environment $\Gamma$, states $s_1 \models \Gamma$ and $s_2 \models \Gamma$ are $\ell$-equal for level $\ell$ (written $s_1 \approx_{\ell} s_2$), if they differ only for variables of a level strictly higher than $\ell$:
	$$s_1 \approx_{\ell} s_2 \deq \forall x:(\tau, \ell') \in \Gamma. \left( \ell' \leq \ell \implies s_1(x) = s_2(x) \right)$$
\end{definition}

\begin{lemma}[Noninterference of $\vdash$]~\\ \label{lem:noninterf} Suppose $s_1 \models \Gamma$, $s_2 \models \Gamma$, and $s_1 \approx_{\ell} s_2$ for some $\ell$. Then for SlicStan statement $S$ and expression $E$:
	\begin{enumerate}
		\item If $~\Gamma \vdash E:(\tau,\ell)$ and $(s_1, E) \Downarrow V_1$ and $(s_2, E) \Downarrow V_2$ then $V_1 = V_2$. 
		\item If $~\Gamma \vdash S:\ell$ and $(s_1, S) \Downarrow s_1', w_1$ and $(s_2, S) \Downarrow s_2', w_2$ then $s_1' \approx_{\ell} s_2'$.
	\end{enumerate}
\end{lemma}

\begin{proof} (1)~follows by rule induction on the derivation $\Gamma \vdash E:(\tau, \ell)$, and using that if $\Gamma \vdash E:(\tau, \ell)$, $x \in \readset(E)$ and $\Gamma(x) = (\tau', \ell')$, then $\ell' \leq \ell$. (2)~follows by rule induction on the derivation $\Gamma \vdash S:\ell$ and using (1).
\end{proof}

% \subsection{Density Semantics} \label{ssec:standen}
% The semantic aspect of a SlicStan 
% program $\Gamma, S$ that we are the most interested in is the final weight $w$
% obtained after evaluating the program $S$.
% This is the value the program computes for the
% unnormalised joint density $p^*(\data,\params, \quants)$ over the 
% data $\data$,
% the model parameters $\params$, and generated quantities $\quants$
% of the program.
% %
% Given a program $\Gamma, S$, we separate the typing environment 
% $\Gamma$ into disjoint parts: $\Gamma_{\sigma}$ and $\Gamma_{\mathbf{x}}$,
% such that $\Gamma_{\sigma}$ contains precisely the variables that are assigned 
% in $S$ and $\Gamma_{\mathbf{x}}$ contains those which never get assigned: %\vspace{-12pt}
% \begin{align*}
% 	\Gamma_{\sigma}=\{(x:T)\in \Gamma\mid x\in W(S)\}\qquad
% 	\Gamma_{\mathbf{x}}=\Gamma\setminus \Gamma_{\sigma}.
% \end{align*}
% Similarly, any conforming state $s\models \Gamma$ separates as $\sigma \uplus \mathbf{x}$
% with 
% \begin{align*}
% 	\sigma =\{(x\mapsto V)\in s\mid x\in W(S)\}\quad \mathbf{x}=s\setminus \sigma.
% \end{align*}
% Then, $\sigma\models \Gamma_{\sigma}$ and $\mathbf{x}\models \Gamma_{\mathbf{x}}$.

% The semantics of a SlicStan program $\Gamma_{\sigma}, \Gamma_{\mathbf{x}}, S$ is a function $\sem{S}$ on states $\sigma \models \Gamma_{\sigma}$ and $\mathbf{x} \models \Gamma_{\mathbf{x}}$, that yields a pair of a state $\sigma'$ and a weight $w$, such that:\vspace{-6pt}
% $$\sem{S}(\sigma)(\mathbf{x}) = \sigma', w, 
% \quad\text{ where } \sigma \uplus \mathbf{x}, S \Downarrow \sigma'\uplus \mathbf{x}, w$$

% We will sometimes refer only to one of the two elements of the pair $\sigma, w$. In those cases we use the notation:
% $\sems{S}(\sigma)(\mathbf{x}),\semp{S}(\sigma)(\mathbf{x})=\sem{S}(\sigma)(\mathbf{x})$.
% We call $\sems{S}$ the \emph{state semantics} and $\semp{S}$ the \emph{density semantics} of $\Gamma, S$.
% We will be particularly interested in the density semantics.

% The function $\semp{S}(\sigma)$ is some positive function $\phi$ on the parameters $\mathbf{x}$.
% % an unnormalised density\footnotemark on $\mathbf{x}$.
% If $\mathbf{x}_1, \mathbf{x}_2$ is a partitioning of $\mathbf{x}$ and $\int \phi(\mathbf{x}) \dif \mathbf{x}_1$ is finite, we say $\phi(\mathbf{x})$ is an unnormalised density $p(\mathbf{x}_1 \mid \mathbf{x}_2) = \phi(\mathbf{x}) /  \int \phi(\mathbf{x}) \dif \mathbf{x}_1$ and we write $\semp{S}(\sigma){\mathbf{x}} \propto p(\mathbf{x}_1 \mid \mathbf{x}_2)$.
% %
% %Given an unnormalized density $f(X,Y)$, we write 
% %$p(X\mid Y)\propto f(X,Y)$ if $p(X\mid Y)=f(X,Y)/\int f(X,Y)\dif X$.
% %In case $\semp{S}(\sigma)(\mathbf{x})$ is normalisable, we write its normalisation $p(\mathbf{x}|\sigma)\propto \semp{S}(\sigma)(\mathbf{x})$.
% Sometimes, when $\sigma$ is clear from context, we will leave it implicit and 
% simply write $p(\mathbf{x})$ for $p(\mathbf{x}; \sigma)$.

% Next, we observe how the state and density semantics compose.

% \begin{lemma}[Semantics composes] \label{lem:sem_properties}~
% 	The state and density semantics compose as follows:
% $$\sems{S_1; S_2}(\sigma)(\mathbf{x}) = \sems{S_2}(\sems{S_2}(\sigma)(\mathbf{x}))(\mathbf{x}) \qquad
% \semp{S_1; S_2}(\sigma)(\mathbf{x}) = \semp{S_1}(\sigma)(\mathbf{x}) \times \semp{S_2}(\sems{S_1}(\sigma)(\mathbf{x}))(\mathbf{x})$$

% \end{lemma}



% Throughout the paper we use the following notation to separate the store in a concise way. 
% \begin{definition}[$\Gamma_{\ell}(s)$ or $s_{\ell}$] ~\\
% For a typing environment $\Gamma$ and a store $s \models \Gamma$, let $\Gamma_{\ell}(s) = \{x \mapsto V \in s \mid \Gamma(x) = (\_, \ell)\}$. When it is clear which typing environment the notation refers to, we write simply $s_{\ell}$ instead of $\Gamma_{\ell}(s)$. 
% \end{definition}

% Using this definition, we re-state the noninterference result in the following  convenient form.
% \begin{lemma}[Noninterference of $\vdash$ reformulated] \label{lem:noninterf-reform}~
% Let $~\Gamma_{\sigma}, \Gamma_{\mathbf{x}}\vdash S$ be a well-typed SlicStan program.
% For all levels $\ell \in \{\lev{data}, \lev{model}, \lev{genquant}\}$, there exist unique functions $f_{\ell}$, such that for all 
% $\sigma \models \Gamma_{\sigma}$, $\mathbf{x} \models \Gamma_{\mathbf{x}}$ and $\sigma'$ such that $\sems{S}(\sigma)(\mathbf{x}) = \sigma'$,
% %
% \quad $ \sigma_{\ell}' = f_{\ell}(\{ \sigma_{\ell'}, \mathbf{x}_{\ell'} \mid \ell' \leq \ell \})$.
% %
% %$$\sems{S}(\sigma)(\mathbf{x}) = \sigma' \quad \implies \quad  
% %\sigma_{\lev{d}}' = f(\sigma_{\lev{d}}, \mathbf{x}_{\lev{d}}), \hquad
% %\sigma_{\lev{m}}' = g(\sigma_{\lev{d}},\sigma_{\lev{m}}, \mathbf{x}_{\lev{d}},  \mathbf{x}_{\lev{m}}), \hquad
% %\sigma_{\lev{q}}' = h(\sigma, \mathbf{x})
% %$$
% \end{lemma}


% % \begin{definition}{Proportionality}
% % 	For random variables $X$ and $Y$, 
% % 	say that $p(X|Y) \propto f(X, Y)$ if there exists a function $c(Y)$ such that $p(X|Y) = c(Y)^{-1} f(X, Y).$ 
% % \end{definition}

\subsection{Shredding and Translation to Stan} \label{ssec:shred}
A key aim of SlicStan is to rearrange the input program into three phases of execution,
corresponding to the levels of the type system: $\lev{data}$ preprocessing, core $\lev{model}$ code to run MCMC or another inference algorithm on, and $\lev{genquant}$, or generated quantities,
which amount to sample post-processing after inference is performed.
The motivation for these phases is that they all naturally appear in the workflow of probabilistic programming.
The blocks of the Stan are built around this phase distinction, and compilation 
of SlicStan to Stan and comparable back-ends requires it.

%Furthermore, the shredding facilitates both a flexible programming style and optimized code generation.
The phases impose different restrictions on the code and make it incur differing computational costs.
The model phase is by far the most expensive to evaluate: code in this phase tends to be executed repeatedly within the inner loop of an inference algorithm like an MCMC method.
Further, it tends to be automatically differentiated \cite{griewank2008evaluating} in case gradient-based inference algorithms are used, which restricts the available programming features and increases the space and time complexity of evaluation.
Type inference in SlicStan combined with shredding allows the user to write their code 
without worrying about the performance of different phases, as 
code will be shredded into its optimal phase of execution.


The shredding relation is in the core of this rearrangement.
Shredding takes a SlicStan statement $S$ and splits it into three \textit{single-level statements} (\autoref{def:singlelev}).
%
That is, $S \shred S_D, S_M, S_Q$ means we split $S$ into sub-statements $S_D, S_M, S_Q$, were $S_D$ mentions only \lev{data} variables, $S_M$ mentions \lev{data} and \lev{model} variables, and $S_Q$ is the rest of the program, and such that the composition $S_D; S_M; S_Q$ behaves the same as the original program $S$. 
When combined with type inference, shredding automatically determines optimal statement placement, such that only necessary work is executed in the `heavy-weight' \lev{model} part of inference.

\begin{display}[.3]{Shredding Relation}
	\clause{S \shred \shredded}{statement shredding} 
\end{display}

We adapt the shredding from \cite{SlicStanPOPL}, so that the following holds for the three sub-statements of a shredded well-typed SlicStan program $\Gamma\vdash S$:
\begin{itemize}
\item $S_D$ implements \textit{deterministic data preprocessing}: no 
contributions to the density are allowed. 
\item $S_M$ is the \textit{inference core}: it is the least restrictive of the three slices --- either or both of $S_D$ and $S_Q$ can be merged into $S_M$. It can involve 
contributions to the density which require advanced inference for sampling. Therefore, this is the part of the program which requires the most computation during inference (in Stan, what is run inside HMC);
\item $S_Q$ represents \textit{sample post-processing}: any contributions to the  density are generative. That is, they can immediately be implemented 
using draws from random number generators.
\end{itemize}
In terms of inference, we can run $S_D$ once as a pre-processing step. Then use a suitable inference algorithm for $S_M$ (in the case of Stan, that's HMC, but we can use other MCMC or VI algorithms) and finally, use ancestral sampling for $S_Q$.

\begin{figure*}
\scalebox{0.81}{\parbox{1.3\linewidth}{%
	\staterule{Shred Assign}
	{\Gamma(L) = (\_,\lev{data}) \rightarrow S_D = L = E, S_M = S_Q = \kw{skip}) \\
     \Gamma(L) = (\_,\lev{model}) \rightarrow S_M = L = E, S_D = S_Q = \kw{skip}) \\
	 \Gamma(L) = (\_,\lev{genquant}) \rightarrow S_Q = L = E, S_D = S_M = \kw{skip})	}
	{ L = E \shred (S_D, S_M, S_Q)}\quad%
	%
	\staterule{Shred Seq}
	{ S_1 \shred S_{D_1}, S_{M_1}, S_{Q_1} \quad 
		S_2 \shred S_{D_2}, S_{M_2}, S_{Q_2}}
	{ S_1; S_2 \shred (S_{D_1};S_{D_2}), (S_{M_1};S_{M_2}), (S_{Q_1};S_{Q_2})  } \qquad%
	%
	\staterule{Shred Skip}
	{}
	{\kw{skip} \shred (\kw{skip}, \kw{skip}, \kw{skip})}\qquad
	%
	%\\[\GAP]\squad
	
	\staterule{Shred Factor}
	{\Gamma(E) = (\_,\lev{data}) \rightarrow S_D = \kw{factor}(E), S_M = S_Q = \kw{skip}) \\
     \Gamma(E) = (\_,\lev{model}) \rightarrow S_M = \kw{factor}(E), S_D = S_Q = \kw{skip}) \\
	 \Gamma(E) = (\_,\lev{genquant}) \rightarrow S_Q = \kw{factor}(E), S_D = S_M = \kw{skip})	}
	{ \kw{factor}(E) \shred (S_D, S_M, S_Q)}\quad\quad
%	
%
	\staterule{Shred Sample}
	{\Gamma(L, E_1, \dots, E_n) = (\_,\lev{data}) \rightarrow S_D = L \sim d(E_1, \dots, E_n), S_M = S_Q = \kw{skip}) \\
	 \Gamma(L, E_1, \dots, E_n) = (\_,\lev{model}) \rightarrow S_M = L \sim d(E_1, \dots, E_n), S_D = S_Q = \kw{skip}) \\
	 \Gamma(L, E_1, \dots, E_n) = (\_,\lev{genquant}) \rightarrow S_Q = L \sim d(E_1, \dots, E_n), S_D = S_M = \kw{skip})	}
	{ L \sim d(E_1, \dots, E_n) \shred (S_D, S_M, S_Q)}\quad\quad
	%
	%\\[\GAP]\squad	
	\staterule{Shred If}
	{   S_1 \shred \shredded[1] \quad 
		S_2 \shred \shredded[2] \quad}
	{ \kw{if}(g)\; S_1\; \kw{else}\; S_2 \shred  
		(\kw{if}(g)\; S_{D_1}\; \kw{else}\; S_{D_2}),  
		(\kw{if}(g)\; S_{M_1}\; \kw{else}\; S_{M_2}), 
		(\kw{if}(g)\; S_{Q_1}\; \kw{else}\; S_{Q_2})}\,% \qquad	
	%
	%\\[\GAP]\squad
	\staterule{Shred For}
	{   S \shred \shredded  }
	{ \kw{for}(x\;\kw{in}\;g_1:g_2)\;S \shred  
		(\kw{for}(x\;\kw{in}\;g_1:g_2)\;S_D),  
		(\kw{for}(x\;\kw{in}\;g_1:g_2)\;S_M), 
		(\kw{for}(x\;\kw{in}\;g_1:g_2)\;S_Q)}%
}}
\end{figure*}

The \ref{Shred If} and \ref{Shred For} rules make sure to shred if and for statements so that they are separated into parts which can be computed independently at each of the three levels. Notice the usage of if and for guards is simplified, to avoid stating rules for when the guard(s) are of different levels (e.g. in $\kw{if}(E)~S_1~\kw{else}~S_2$, if $E$ is of level \lev{model}, the first bit of shredding must be \kw{skip}, as we cannot access $E$).

These shredding rules follow very closely those given by \citet{SlicStanPOPL}. The main difference is that sample statements ($L \sim d(E_1, \dots, E_n)$) are allowed to be of \lev{genquant} and can be included in the last, generative slice of the program (see rule \ref{Shred Sample}).

We provide proofs for the following key results in \autoref{ap:proofs}: shredding produces \textit{single-level statements} (\autoref{def:singlelev} 
and \autoref{lem:shredisleveled}) and shredding is semantic preserving (Lemma~\ref{lem:shred}).

Intuitively, a single-level statement of level $\ell$ is one that updates only variables of level $\ell$. 
\begin{definition}[Single-level Statement $\Gamma \vdash \ell(S)$] \label{def:singlelev}
	~\\
	We define single-level statements  $S$ of level $\ell$ with respect to $\Gamma$ (written $\Gamma \vdash \ell(S)$), informally, to be statements which only contain writes to variables which are of level $\ell$ in $\Gamma$
	\emph{and} which only contain $\kw{factor}(E)$ and $L\sim d(E_1,\ldots,E_n)$ statements which type-check 
	at level $\ell$ but not at any $\ell'<\ell$.
	For a precise definition, see \autoref{ap:proofs}.
\end{definition}

\begin{lemma}[Shredding produces single-level statements] \label{lem:shredisleveled}
	%\todo{Extend to if and only if : where do we need it to be iff again?}
	$$\Gamma\vdash S \;\wedge\;
	S \shred[\Gamma] \shredded \implies 
	\singlelevelS{\lev{data}}{S_D} \wedge \singlelevelS{\lev{model}}{S_M} \wedge \singlelevelS{\lev{genquant}}{S_Q}$$
\end{lemma}

%\begin{lemma}[Single-level statements only change part of the store] \label{lem:single-level-store} ~ \\
%If $~\Gamma \vdash \ell(S)$, then for all $\sigma, \mathbf{x} \models \Gamma_{\sigma}, \Gamma_{\mathbf{x}}$ and $\sigma'$ such that $\sems{S}(\mathbf{x}) = \sigma'$, we have:
%$$\sigma_{\ell'} = \sigma_{\ell'}' \text{ for all } \ell' \neq \ell$$
%\end{lemma}

We prove a result about the effect of single-level statements on the store and weight of well-typed programs:
\begin{lemma}[Property of single-level statements] \label{lem:single-lev-prop} ~\\
	Let $~\Gamma_{\sigma}, \Gamma_{\mathbf{x}}, S$ be SlicStan program, such that $S$ is single-level statement of level $\ell$, $\Gamma \vdash \ell(S)$. Then there exist unique functions $f$ and $\phi$, such that for any $\sigma, \mathbf{x} \models \Gamma_{\sigma}, \Gamma_{\mathbf{x}}$: 
	$$  \sem{S}(\sigma)(x) = f(\sigma_{\leq \ell}, \mathbf{x}_{\leq \ell})\cup \sigma_{> \ell} , \hquad \phi(\sigma_{\leq \ell})(\mathbf{x}_{\leq \ell}), $$
	where we write $\sigma_{\leq \ell}=\{(x\mapsto V)\in \sigma\mid \Gamma_{\sigma}(x)=(\_,\ell)\}$ and $\sigma_{>\ell}=\sigma\setminus \sigma_{\leq \ell}$.
\end{lemma}

\begin{lemma}[Semantic Preservation of $\shred$] \label{lem:shred} ~ \\
	If $~\Gamma \vdash S:\lev{data} $ and $ S \shred[\Gamma] \shredded $ then $\sem{S} = \sem{S_D; S_M; S_Q}$.
\end{lemma}
% \subsection{Density Factorisation}
% As an extension of \cite{SlicStanPOPL},
% we show that shredding induces a natural factorization of the density 
% implemented by the program: $p(\data, \params, Q) = p(\params,\data)p(Q \mid \params,\data)$.
% This means that we can separate the program into a deterministic preprocessing part, a part that uses a `heavy-weight' inference algorithm, such as HMC, and a part that uses simple ancestral sampling. 

% \begin{theorem}[Shredding induces a factorisation of the density]\label{th:shred_gen}~ \\
% 	Suppose $\Gamma \vdash S : \lev{data}$ and $~S \shred[\Gamma] S_D, S_M, S_Q$
% 	and $\Gamma = \Gamma_{\sigma} \cup \Gamma_{\data} \cup \Gamma_{\params} \cup \Gamma_{\quants}$.
% 	% $\sems{S_Q}(\sigma_M)(\data, \params, \quants) = \sigma_Q$.
% 	%
% 	For all $\sigma$, $\data$, $\params$, and $\quants$:
% 	if $\sigma, \data, \params, \quants \models \Gamma_{\sigma}, \Gamma_{\data}, \Gamma_{\params}, \Gamma_{\quants}$,
% 	and $\semp{S}(\sigma)(\data, \params, \quants) \propto p(\data, \params, Q)$
% 	and  $\tildeset(S_Q)=\dom(\Gamma_Q)$ then:
% 	\begin{enumerate}
% 		%\item $\semp{S_D}(\sigma)(\data, \params, \quants) = 1$
% 		\item $\semp{S_M}(\sigma_D)(\data, \params, \quants) \propto p(\params, \data)$
% 		\item $\semp{S_Q}(\sigma_M)(\data, \params, \quants) = p(Q \mid \params, \data)$
% 	\end{enumerate}
% 	where $\sigma_D = \sems{S_D}(\sigma)(\data, \params, \quants)$
% 	and $\sigma_M = \sems{S_M}(\sigma_D)(\data, \params, \quants)$
% 	and $p(\data, \params, Q) = p(\data, \params)p(Q \mid \data, \params)$.
% \end{theorem}
% \begin{proof}
% This follows by proving a more general result using induction on the structure of $S$, \autoref{lem:shred}, \autoref{lem:sem_properties} and \autoref{lem:shredisleveled}. See \autoref{ap:proofs} for full proof.
% \end{proof}

% The given SlicStan program $S$ defines a joint density $p(\data, \params, Q)$.
% By shredding we obtain a \lev{model} block $S_M$ that defines $p(\params, \data)$
% and a \lev{genquant} block $S_Q$ that defines $p(Q \mid \params, \data)$.
% Hence, inference in Stan using these blocks recovers the semantics $p(\data, \params, Q)$ of the SlicStan program.


